Facilitating a 3D granular flow with an obstruction

Ensuring a smooth rate of efflux of particles from an outlet without unpredictable clogging events is crucial in processing powders and grains. We show by experiments and simulations that an obstacle placed near the outlet can greatly suppress clog formation in a 3-dimensional granular flow; this counterintuitive phenomenon had previously been demonstrated in 2-dimensional systems. Remarkably, clog suppression is very effective even when the obstacle cross-section is comparable to that of a single grain, and is only a small fraction of the outlet area. Data from two dissimilar obstacle shapes indicate that the underlying mechanism for clog suppression is geometric: while the magnitude of the effect can be affected by dynamical factors, the optimal location of the obstacle is determined entirely by a simple geometric rule. An optimally-placed obstacle arranges for the most-probable clogging arch to be at a perilous and unstable spot, where the local flow geometry is at a point of expansion and a slight perturbation leaves the arch without downstream support. This geometric principle does not rely on previously conjectured dynamical mechanisms and admits generalization to other agent-based and particulate systems.

==> latexmkrc <==
$sub_doc_output = 'output-subdoc';

@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne '') && ($sub_doc_output ne '.') ) {

             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}
